Complete NNLO Operator Bases in Higgs Effective Field Theory

For the first time, we list the complete and independent set of operators at the next-to-next-to-leading order (NNLO) in the Higgs effective field theory (HEFT), also named as the electroweak chiral Lagrangian with the light Higgs boson. The Young tensor technique utilized in this work guarantees the completeness and independence of the on-shell amplitude basis while the Adler zero condition imposes non-linear symmetry on the Nambu-Goldstone bosons that play the central role in the chiral Lagrangian. The spurion fields are incorporated into the gauge structure of operators following the Littlewood-Richardson rule to accommodate custodial symmetry breaking. We enumerate 11506 (1927574) NNLO operators for one (three) flavor of fermions for the electroweak chiral Lagrangian with the light Higgs. Below the electroweak symmetry breaking scale, the dimension-8 standard model effective field theory (SMEFT) operators could be matched to these HEFT operators at both the NLO and NNLO orders.

==> 6_pis2D.tex <==
\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{6}{*}{$ {L_L}{L^\dagger_R}^2\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{i}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{i}}({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{i}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{i}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{i}}({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {L_L}{L^\dagger_R}^2{\mathbf{T}}\phi{L_R} D$} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{i}}{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{i}}{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{i}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{l}}{{\tau^{J}}_{k}^{i}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{i}}{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{i}}{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{l}}{{\tau^{J}}_{k}^{i}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{7}{*}{$ {L_L}{L^\dagger_R}^2{\mathbf{T}}^2\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{j}^{i}}{{\tau^{M}}_{k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{j}^{i}}{{\tau^{M}}_{k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{j}^{l}}{{\tau^{M}}_{k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{j}^{i}}{{\tau^{M}}_{k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{j}^{i}}{{\tau^{M}}_{k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{j}^{l}}{{\tau^{M}}_{k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\

\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{1}{*}{$ {L_L}{L^\dagger_R}^2{\mathbf{T}}^2\phi{L_R}D $}
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
$ {L_L}{L^\dagger_R}^2{\mathbf{T}}^3\phi{L_R}D $ & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{6}{*}{$ {L_L}^2{L^\dagger_R}\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {L_L}^2{L^\dagger_R}{\mathbf{T}}\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_ {l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_ {l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{j}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{5}{*}{$ {L_L}^2{L^\dagger_R}{\mathbf{T}}^2\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\

\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{3}{*}{$ {L_L}^2{L^\dagger_R}{\mathbf{T}}^2\phi{L^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{i}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L_L}^2{L^\dagger_R}{\mathbf{T}}^3\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}{{{L^\dagger_R}_{s}}^{k}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{6}{*}{$ {L_L}{L^\dagger_R}^2h{L_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}{L^\dagger_R}^2h{\mathbf{T}}{L_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{k}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{k}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}})({{{L_R}_{t}}_{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{3}{*}{$ {L_L}{L^\dagger_R}^2h{\mathbf{T}}^2{L_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{k}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{2}{*}{$ {L_L}^2{L^\dagger_R}h{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\

\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{4}{*}{$ {L_L}^2{L^\dagger_R}h{L^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]h({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]h({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}^2{L^\dagger_R}h{\mathbf{T}}{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{j}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{i}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{i}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{k}})) $ \\
\hline
\multirow{3}{*}{$ {L_L}^2{L^\dagger_R}h{\mathbf{T}}^2{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L_L}_{r}}_{j}}){{{L^\dagger_R}_{s}}^{k}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L_L}_{r}}_{j}}({D_{\mu}}{{{L^\dagger_R}_{s}}^{k}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_L}_{r}}_{j}}{\sigma^{\nu\mu}}{{{L^\dagger_R}_{s}}^{k}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{6}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}\phi{Q_R}D $} & $ {{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{3}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}{\mathbf{T}}\phi{Q_R}D $} & $ {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{9}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}{\mathbf{T}}\phi{Q_R}D $}
 & $ {{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{8}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}{\mathbf{T}}^2\phi{Q_R}D $} & $  {{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}{\mathbf{T}}^3\phi{Q_R}D $} & $ {{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{6}{*}{$ {L_L}{L^\dagger_R}{Q_L}\phi{Q^\dagger_L}D $} & $ {{\tau^{I}}_ {j}^{i}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{i}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{k}}({{{Q^\dagger_L}_{t}}^{ai}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{k}}({{{Q^\dagger_L}_{t}}^{ai}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{i}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{i}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{aj}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{12}{*}{$ {L_L}{L^\dagger_R}{Q_L}{\mathbf{T}}\phi{Q^\dagger_L}D $} & $ {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {l}^{k}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {l}^{k}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {j}^{k}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {j}^{k}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{k}}{{\tau^{J}}_ {l}^{i}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {j}^{k}}{{\tau^{J}}_ {l}^{i}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{k}}{{\tau^{J}}_ {j}^{i}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {l}^{k}}{{\tau^{J}}_ {j}^{i}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {l}^{k}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {l}^{k}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{8}{*}{$ {L_L}{L^\dagger_R}{Q_L}{\mathbf{T}}^2\phi{Q^\dagger_L}D $} & $  {{\tau^{K}}_ {l}^{k}}{{\tau^{M}}_ {j}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{K}}_ {l}^{k}}{{\tau^{M}}_ {j}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {l}^{k}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {l}^{k}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {l}^{k}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {l}^{k}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {l}^{i}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {l}^{i}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{aj}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L_L}{L^\dagger_R}{Q_L}{\mathbf{T}}^3\phi{Q^\dagger_L}D $} & $ {{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {j}^{k}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {j}^{k}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{3}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}\phi{L_R}D $} & $ {{\tau^{I}}_ {i}^{j}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {i}^{j}}({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {k}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{3}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}\phi{L_R}D $}
 & $ {{\tau^{I}}_ {k}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {i}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {i}^{l}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}{\mathbf{T}}\phi{L_R}D $} & $ {{\tau^{K}}_ {k}^{l}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {k}^{l}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {k}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_ {k}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{i}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {i}^{l}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {i}^{l}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L_R}_{t}}_{i}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {k}^{j}}{{\tau^{J}}_ {i}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_ {k}^{j}}{{\tau^{J}}_ {i}^{l}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{8}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}{\mathbf{T}}^2\phi{L_R}D $} & $  {{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{i}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{K}}_ {k}^{j}}{{\tau^{M}}_ {i}^{l}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{K}}_ {k}^{j}}{{\tau^{M}}_ {i}^{l}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {i}^{j}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {i}^{j}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}{\mathbf{T}}^3\phi{L_R}D $} & $ {{\tau^{J}}_ {i}^{l}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{J}}_ {i}^{l}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{6}{*}{$ {L_L}{Q_L}{Q^\dagger_R}\phi{L^\dagger_L}D $} & $ {{\tau^{I}}_{l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{l}^{i}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{i}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{i}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{j}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{j}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {L_L}{Q_L}{Q^\dagger_R}{\mathbf{T}}\phi{L^\dagger_L}D $} & $ {{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ {{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 \hline
\multirow{7}{*}{$ {L_L}{Q_L}{Q^\dagger_R}{\mathbf{T}}^2\phi{L^\dagger_L}D $} & $  {{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $  {{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{1}{*}{$ {L_L}{Q_L}{Q^\dagger_R}{\mathbf{T}}^2\phi{L^\dagger_L}D $}
 & $  {{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L_L}{Q_L}{Q^\dagger_R}{\mathbf{T}}^3\phi{L^\dagger_L}D $} & $ \

{{\tau^{J}}_{l}^{i}}{{\tau^{K}}_{k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $
 {{\tau^{J}}_{l}^{i}}{{\tau^{K}}_{k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{6}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}h{Q_R}D $} & $ ({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ h({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ h({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{Q_R}_{t}}_{aj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ ({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ h({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ h({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q_R}_{t}}_{ak}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}h{\mathbf{T}}{Q_R}D $} & $ {{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{aj}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q_R}_{t}}_{aj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q_R}_{t}}_{ak}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{3}{*}{$ {L_L}{L^\dagger_R}{Q^\dagger_R}h{\mathbf{T}}^2{Q_R}D $} & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q_R}_{t}}_{al}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{4}{*}{$ {L_L}{L^\dagger_R}{Q_L}h{Q^\dagger_L}D $} & $ ({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{Q_L}_{s}}_{ak}}) $ \\
 & $ h({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{Q_L}_{s}}_{ak}})) $ \\
 & $ h({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}})({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ ({{{Q^\dagger_L}_{t}}^{ai}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q_L}_{s}}_{aj}}) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{2}{*}{$ {L_L}{L^\dagger_R}{Q_L}h{Q^\dagger_L}D $}
 & $ h({{{Q^\dagger_L}_{t}}^{ai}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q_L}_{s}}_{aj}})) $ \\
 & $ h({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{aj}})({{{Q^\dagger_L}_{t}}^{ai}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}{L^\dagger_R}{Q_L}h{\mathbf{T}}{Q^\dagger_L}D $} & $ {{\tau^{I}}_ {l}^{k}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{i}}){{{Q_L}_{s}}_{ak}}) $ \\
 & $ {{\tau^{I}}_ {l}^{k}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{i}}({D_{\mu}}{{{Q_L}_{s}}_{ak}})) $ \\
 & $ {{\tau^{I}}_ {l}^{k}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{i}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}})({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q_L}_{s}}_{aj}}) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q_L}_{s}}_{aj}})) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{aj}})({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q_L}_{s}}_{ak}}) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q_L}_{s}}_{ak}})) $ \\
 & $ {{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}})({{{Q^\dagger_L}_{t}}^{ak}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{3}{*}{$ {L_L}{L^\dagger_R}{Q_L}h{\mathbf{T}}^2{Q^\dagger_L}D $} & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {l}^{k}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{L^\dagger_R}_{r}}^{j}}){{{Q_L}_{s}}_{ak}}) $ \\
 & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {l}^{k}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{L^\dagger_R}_{r}}^{j}}({D_{\mu}}{{{Q_L}_{s}}_{ak}})) $ \\
 & $  {{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {l}^{k}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_R}_{r}}^{j}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ak}})({{{Q^\dagger_L}_{t}}^{al}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{6}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}h{L_R}D $} & $ ({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{ai}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ h({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ h({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
 & $ ({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ h({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ h({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{L_R}_{t}}_{i}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
\hline
\multirow{5}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}h{\mathbf{T}}{L_R}D $} & $ {{\tau^{I}}_ {k}^{j}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{j}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{i}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{j}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L_R}_{t}}_{i}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
 & $ {{\tau^{I}}_ {i}^{j}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {i}^{j}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{k}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{4}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}h{\mathbf{T}}{L_R}D $}
 & $ {{\tau^{I}}_ {i}^{j}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L_R}_{t}}_{k}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
 & $ {{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{ai}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
\hline
\multirow{3}{*}{$ {L^\dagger_R}{Q_L}{Q^\dagger_R}h{\mathbf{T}}^2{L_R}D $} & $ {{\tau^{I}}_ {i}^{l}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {i}^{l}}{{\tau^{J}}_ {k}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {i}^{l}}{{\tau^{J}}_ {k}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L^\dagger_R}_{p}}^{i}})) $ \\
\hline
\multirow{6}{*}{$ {L_L}{Q_L}{Q^\dagger_R}h{L^\dagger_L}D $} & $ ({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ h({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ h({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ ({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ h({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ h({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{L^\dagger_L}_{t}}^{i}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}{Q_L}{Q^\dagger_R}h{\mathbf{T}}{L^\dagger_L}D $} & $ {{\tau^{I}}_ {l}^{j}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ {{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ {{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ {{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L^\dagger_L}_{t}}^{j}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{3}{*}{$ {L_L}{Q_L}{Q^\dagger_R}h{\mathbf{T}}^2{L^\dagger_L}D $} & $ {{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ {{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{12}{*}{$ {L^\dagger_R}{Q^\dagger_R}^2{\mathbf{T}}\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{i}^{m}}{{\tau^{J}}_{j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{i}^{m}}{{\tau^{J}}_{j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_{j}^{m}}{{\tau^{J}}_{i}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{i}^{m}}{{\tau^{J}}_{j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{i}^{m}}{{\tau^{J}}_{j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_{j}^{m}}{{\tau^{J}}_{i}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{8}{*}{$ {L^\dagger_R}{Q^\dagger_R}^2{\mathbf{T}}^2\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{i}^{m}}{\epsilon_{abc}}{\epsilon_{jk}}{\epsilon_{lm}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_{i}^{m}}{\epsilon_{abc}}{\epsilon_{jl}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_{i}^{m}}{{\tau^{M}}_{j}^{n}}{\epsilon_{abc}}{\epsilon^{IJM}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{i}^{m}}{\epsilon_{abc}}{\epsilon_{jk}}{\epsilon_{lm}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}_{\nu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_{i}^{m}}{\epsilon_{abc}}{\epsilon_{jl}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_{i}^{m}}{{\tau^{M}}_{j}^{n}}{\epsilon_{abc}}{\epsilon^{IJM}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L^\dagger_R}{Q^\dagger_R}^2{\mathbf{T}}^3\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {i}^{m}}{{\tau^{K}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{m}}{{\tau^{K}}_ {i}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{3}{*}{$ {Q^\dagger_R}^3{\mathbf{T}}\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{K}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{K}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\

 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{5}{*}{$ {Q^\dagger_R}^3{\mathbf{T}}\phi{L^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{K}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{jk}}{{\mathbf{T}}^{I}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{K}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon^{IJK}}{\epsilon_{ik}}{\epsilon_{lm}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{5}{*}{$ {Q^\dagger_R}^3{\mathbf{T}}^2\phi{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{J}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr,s}]{{\tau^{J}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr,s}]{{\tau^{J}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}_{\nu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr,s}]{{\tau^{K}}_ {i}^{m}}{{\tau^{M}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon^{IJM}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r,s}]{{\tau^{J}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon_{il}}{\epsilon_{km}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
$ {Q^\dagger_R}^3{\mathbf{T}}^3\phi{L^\dagger_L}D $ & $ \mathcal{Y}[\ytableaushort{pr,s}]{{\tau^{J}}_ {i}^{m}}{{\tau^{K}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{3}{*}{$ {L^\dagger_R}{Q^\dagger_R}^2h{\mathbf{T}}^2{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {i}^{n}}{{\tau^{J}}_ {j}^{m}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{cl}}{\bar{\sigma}^{\mu}}{{{L^\dagger_R}_{p}}^{i}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{bk}}) $ \\
\hline
\multirow{2}{*}{$ {Q^\dagger_R}^3h{\mathbf{T}}^2{L^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{bj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr,s}]{{\tau^{I}}_ {i}^{m}}{{\tau^{J}}_ {j}^{n}}{\epsilon_{abc}}{\epsilon_{km}}{\epsilon_{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L^\dagger_L}_{t}}^{l}}{\bar{\sigma}^{\mu}}{{{Q^\dagger_R}_{p}}^{ai}})({{{Q^\dagger_R}_{r}}^{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
\hline
\multirow{9}{*}{$ {Q_L}{Q^\dagger_R}^2\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{3}{*}{$ {Q_L}{Q^\dagger_R}^2\phi{Q_R}D $}
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{l}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{22}{*}{$ {Q_L}{Q^\dagger_R}^2{\mathbf{T}}\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {k}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {j}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{2}{*}{$ {Q_L}{Q^\dagger_R}^2{\mathbf{T}}\phi{Q_R}D $}
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{16}{*}{$ {Q_L}{Q^\dagger_R}^2{\mathbf{T}}^2\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{i}}{{\tau^{M}}_ {k}^{l}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{l}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{4}{*}{$ {Q_L}{Q^\dagger_R}^2{\mathbf{T}}^3\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{J}}_ {k}^{i}}{{\tau^{K}}_ {j}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{3}{*}{$ {Q_L}^2{Q^\dagger_R}\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{l}^{i}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{l}^{i}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{i}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{9}{*}{$ {Q_L}^2{Q^\dagger_R}\phi{Q^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{i}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{j}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{j}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{l}^{i}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{l}^{i}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{i}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{i}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{j}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{j}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{16}{*}{$ {Q_L}^2{Q^\dagger_R}{\mathbf{T}}\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_{l}^{i}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{k}^{i}}{{\tau^{J}}_{l}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{8}{*}{$ {Q_L}^2{Q^\dagger_R}{\mathbf{T}}\phi{Q^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_{l}^{i}}{{\tau^{J}}_{k}^{j}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{K}}_{l}^{j}}{\epsilon^{IJK}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{16}{*}{$ {Q_L}^2{Q^\dagger_R}{\mathbf{T}}^2\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{K}}_ {l}^{j}}{{\tau^{M}}_ {k}^{i}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {k}^{j}}{{\tau^{M}}_ {l}^{i}}{\epsilon^{IKM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{K}}_ {l}^{i}}{{\tau^{M}}_ {k}^{j}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{K}}_ {l}^{i}}{{\tau^{M}}_ {k}^{j}}{\epsilon^{IJM}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{1}{*}{$ {Q_L}^2{Q^\dagger_R}{\mathbf{T}}^3\phi{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{3}{*}{$ {Q_L}^2{Q^\dagger_R}{\mathbf{T}}^3\phi{Q^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{J}}_ {l}^{i}}{{\tau^{K}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {Q_L}{Q^\dagger_R}^2h{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ci}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ci}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}})({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{ai}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]h({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ci}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ci}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ci}})({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{ai}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]h({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\multirow{10}{*}{$ {Q_L}{Q^\dagger_R}^2h{\mathbf{T}}{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{ai}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{ai}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{8}{*}{$ {Q_L}{Q^\dagger_R}^2h{\mathbf{T}}{Q_R}D $}
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{ai}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{l}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{ai}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{ck}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {j}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{ck}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\multirow{6}{*}{$ {Q_L}{Q^\dagger_R}^2h{\mathbf{T}}^2{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {j}^{i}}{{\tau^{J}}_ {k}^{l}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q^\dagger_R}_{r}}^{aj}}){{{Q^\dagger_R}_{s}}^{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q^\dagger_R}_{r}}^{aj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {j}^{l}}{{\tau^{J}}_ {k}^{i}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_R}_{r}}^{aj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ck}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\multirow{11}{*}{$ {Q_L}^2{Q^\dagger_R}h{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]h({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]h({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]h({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]h({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{1}{*}{$ {Q_L}^2{Q^\dagger_R}h{Q^\dagger_L}D $}
 & $ \mathcal{Y}[\ytableaushort{p, r}]h({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{Q^\dagger_L}_{t}}^{bi}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\multirow{18}{*}{$ {Q_L}^2{Q^\dagger_R}h{\mathbf{T}}{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{j}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ai}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{j}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ai}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{aj}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{aj}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {l}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{aj}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r}]{{\tau^{I}}_ {k}^{i}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q^\dagger_L}_{t}}^{bj}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\multirow{6}{*}{$ {Q_L}^2{Q^\dagger_R}h{\mathbf{T}}^2{Q^\dagger_L}D $} & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr}]{{\tau^{I}}_ {k}^{i}}{{\tau^{J}}_ {l}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {k}^{j}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q^\dagger_R}_{s}}^{ak}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {k}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q^\dagger_R}_{s}}^{ak}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {l}^{i}}{{\tau^{J}}_ {k}^{j}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q^\dagger_R}_{s}}^{ak}})({{{Q^\dagger_L}_{t}}^{bl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{6}{*}{$ {L_L}{Q_L}^2\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{k}}{\epsilon^{abc}}{\epsilon^{il}}{\epsilon^{jm}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{k}}{\epsilon^{abc}}{\epsilon^{il}}{\epsilon^{jm}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{12}{*}{$ {L_L}{Q_L}^2{\mathbf{T}}\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{K}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{IJK}}{\epsilon^{jk}}{\epsilon^{lm}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{kl}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{k}}{{\tau^{J}}_ {n}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{k}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{il}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{IJK}}{\epsilon^{jk}}{\epsilon^{lm}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{kl}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{k}}{{\tau^{J}}_ {n}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{k}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{il}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{7}{*}{$ {L_L}{Q_L}^2{\mathbf{T}}^2\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {n}^{l}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{im}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {n}^{l}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{im}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{1}{*}{$ {L_L}{Q_L}^2{\mathbf{T}}^2\phi{Q_R}D $}
 & $ \mathcal{Y}[\ytableaushort{p,r}]{{\tau^{J}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{2}{*}{$ {L_L}{Q_L}^2{\mathbf{T}}^3\phi{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{J}}_ {m}^{k}}{{\tau^{K}}_ {n}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{ln}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{K}}_ {n}^{k}}{{\tau^{M}}_ {m}^{i}}{{\tau^{N}}_ {o}^{j}}{\epsilon^{abc}}{\epsilon^{IJN}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}{{\mathbf{T}}^{M}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}{{{Q_L}_{s}}_{bk}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{4}{*}{$ {Q_L}^3\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{kl}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{8}{*}{$ {Q_L}^3{\mathbf{T}}\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{K}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{IJK}}{\epsilon^{jk}}{\epsilon^{lm}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{K}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{IJK}}{\epsilon^{jk}}{\epsilon^{lm}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{\epsilon^{abc}}{\epsilon^{il}}{\epsilon^{jk}}{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{kl}}{\epsilon^{mn}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{K}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{IJK}}{\epsilon^{jk}}{\epsilon^{lm}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{5}{*}{$ {Q_L}^3{\mathbf{T}}^2\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {n}^{l}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{im}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{{\tau^{K}}_ {o}^{k}}{\epsilon^{abc}}{\epsilon^{lm}}{\epsilon^{no}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{1}{*}{$ {Q_L}^3{\mathbf{T}}^3\phi{L_R}D $} & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{J}}_ {m}^{k}}{{\tau^{K}}_ {n}^{i}}{\epsilon^{abc}}{\epsilon^{jm}}{\epsilon^{ln}}{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}{{\mathbf{T}}^{K}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}{{{Q_L}_{s}}_{ck}}){{\mathbf{V}^I}_\mu} $ \\
\hline
\multirow{4}{*}{$ {L_L}{Q_L}^2h{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q_L}_{s}}_{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{2}{*}{$ {L_L}{Q_L}^2h{Q_R}D $}
 & $ \mathcal{Y}[\ytableaushort{r, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q_L}_{s}}_{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
\hline
\multirow{9}{*}{$ {L_L}{Q_L}^2h{\mathbf{T}}{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q_L}_{s}}_{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jl}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jl}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q_L}_{s}}_{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{aj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{bk}})({{{Q_R}_{t}}_{cl}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{L_L}_{p}}_{i}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jl}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
\hline
\multirow{3}{*}{$ {L_L}{Q_L}^2h{\mathbf{T}}^2{Q_R}D $} & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{rs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})({{{Q_L}_{r}}_{aj}}({D_{\mu}}{{{Q_L}_{s}}_{bk}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{r,s}]{{\tau^{I}}_ {n}^{i}}{{\tau^{J}}_ {m}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{Q_R}_{t}}_{cl}}{\bar{\sigma}^{\mu}}{{{L_L}_{p}}_{i}})(({D_{\mu}}{{{Q_L}_{r}}_{aj}}){{{Q_L}_{s}}_{bk}}) $ \\
\hline
\multirow{4}{*}{$ {Q_L}^3h{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q_L}_{s}}_{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q_L}_{s}}_{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{\epsilon^{abc}}{\epsilon^{ik}}{\epsilon^{jl}}h({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
\hline
\multirow{6}{*}{$ {Q_L}^3h{\mathbf{T}}{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jl}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{Q_L}_{r}}_{bj}}{\sigma^{\nu\mu}}{{{Q_L}_{s}}_{ck}})({{{L_R}_{t}}_{l}}{\bar{\sigma}_{\nu}}({D_{\mu}}{{{Q_L}_{p}}_{ai}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{\epsilon^{abc}}{\epsilon^{jl}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q_L}_{s}}_{ck}})) $ \\
 & $ \mathcal{Y}[\ytableaushort{p, r, s}]{{\tau^{I}}_ {m}^{l}}{\epsilon^{abc}}{\epsilon^{ij}}{\epsilon^{km}}h{{\mathbf{T}}^{I}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
\hline
\multirow{1}{*}{$ {Q_L}^3h{\mathbf{T}}^2{L_R}D $} & $ \mathcal{Y}[\ytableaushort{prs}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})(({D_{\mu}}{{{Q_L}_{r}}_{bj}}){{{Q_L}_{s}}_{ck}}) $ \\
\hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r|ll}
\hline
\multirow{1}{*}{$ {Q_L}^3h{\mathbf{T}}^2{L_R}D $}
 & $ \mathcal{Y}[\ytableaushort{pr, s}]{{\tau^{I}}_ {m}^{i}}{{\tau^{J}}_ {n}^{j}}{\epsilon^{abc}}{\epsilon^{km}}{\epsilon^{ln}}h{{\mathbf{T}}^{I}}{{\mathbf{T}}^{J}}({{{L_R}_{t}}_{l}}{\bar{\sigma}^{\mu}}{{{Q_L}_{p}}_{ai}})({{{Q_L}_{r}}_{bj}}({D_{\mu}}{{{Q_L}_{s}}_{ck}})) $ \\
\hline
\end{tabular}
\end{center}
